Retracting Graphs to Cycles

We initiate the algorithmic study of retracting a graph into a cycle in the graph, which seeks a mapping of the graph vertices to the cycle vertices, so as to minimize the maximum stretch of any edge, subject to the constraint that the restriction of the mapping to the cycle is the identity map. This problem has its roots in the rich theory of retraction of topological spaces, and has strong ties to well-studied metric embedding problems such as minimum bandwidth and 0-extension. Our first result is an O(min{k, sqrt{n}})-approximation for retracting any graph on n nodes to a cycle with k nodes. We also show a surprising connection to Sperner's Lemma that rules out the possibility of improving this result using natural convex relaxations of the problem. Nevertheless, if the problem is restricted to planar graphs, we show that we can overcome these integrality gaps using an exact combinatorial algorithm, which is the technical centerpiece of the paper. Building on our planar graph algorithm, we also obtain a constant-factor approximation algorithm for retraction of points in the Euclidean plane to a uniform cycle.

==> LP.tex <==
\section{LP}

Consider an arbitrary graph $G$ and subgraph $H$ that is a cycle, an integer $l$.  
Fix a direction for graph $H$. Fix one direction for each edge $e \in E(G)$, such that edges in $H$ have all same direction as direction of $H$. 
For each circulation of a cycle in graph $G$ with length at most $l$ consider a variable $f_{\overrightarrow{C}}$.

Note that by $e \parallel \overrightarrow{C}$ we mean that $e \in E(\overrightarrow{C})$ and $e$ has same direction as $\overrightarrow{C}$, and by $e \nparallel \overrightarrow{C}$, we mean that 
$e \in E(\overrightarrow{C})$, but $e$ has opposite direction of $\overrightarrow{C}$. 

In the following, we have the LP feasibility problem:

\begin{alignat*}{3}
& \text{minimize}   \quad && 0  \quad && \\
& \text{subject to} \quad &&    \quad && \\
&   \quad && \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \parallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} - \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \nparallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} =1 \quad && \forall e \in H \\
&  \quad &&  \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \parallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} - \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \nparallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} = 0   \quad &&  \forall e \notin H \\
& \quad && f_{\overrightarrow{C}} \geq 0  \quad && 
\end{alignat*}


\iffalse
\begin{alignat*}{3} 
 & \text{minimize} \quad && 0  && \\
 & \text{subject to} && && \\  
\quad&\sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \parallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} - \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \nparallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} =1 \qquad \forall e \in H\\
\quad&\sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \parallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} - \sum_{\overrightarrow{C}: e \in \overrightarrow{C},  e \nparallel  \overrightarrow{C} }  
f_{\overrightarrow{C}} = 0 \qquad \forall e \notin H \\
\quad& f_{\overrightarrow{C}} \geq 0 
\end{alignat*}
\fi

Here is the dual of the LP: 
\begin{alignat*}{3}
  & \text{maximize} \quad && \sum_{e \in H} x_e  \quad && \\
  & \text{subject to: } \quad && \quad &&  \\
  & \quad && \sum_{e: e \in \overrightarrow{C}, e \parallel \overrightarrow{C}} x_e - \sum_{e: e \in \overrightarrow{C},  e \nparallel \overrightarrow{C}} x_e = 0 \quad && \forall \overrightarrow{C} 
\end{alignat*}

Note that if we can show that the Dual value is bounded, then it means that the Primal program itself has a feasible solution for a given $l$. On the other hand, if we show that the Dual value is unbounded, then the Primal itself has not any feasible solution. Also note that in this dual program number of constraints is exponential, and in order to solve it we need a separation oracle. Here the question is that is there any polynomial procedure that takes value of $x_e$s and checks whether $x_e$ values satisfy the constraints, and if it does not satisfy, which constraint is violated.  


==> generalizations.tex <==
\section{Generalizations: Hosts, Guests, and Weights}
In this section, we study graph retractions to other classes of hosts, including arbitrary graphs and metrics.  First, we consider the case that the host is a constant-dimensional grid.  We present a polynomial-time algorithm that achieves an $O(d)$-approximate retraction to any $d$-dimensional uniform grid.  Next, we present two results for the case where the host is an arbitrary metric.  In both cases, we assume that there is a weight for each edge of the guest graph and our goal is to minimize the maximum weighted stretch.  We show that if the guest graph has bounded treewidth, then a retraction of optimal weighted stretch can be computed in polynomial time.  Our final result is that if the guest graph is arbitrary, then there is no polynomial-time $O(\log^{1/4} n)$-approximation algorithm for minimizing weighted stretch, unless P = NP.   

==> k_approximation.tex <==
\subsection{k-approximation algorithm}
In this section, we study the problem of retracting an unweighted graph $G$ to a subset $H$ of its vertices called anchors, where the stretch of the retractions is defined based on the distances of a given metric over vertices of $H$. And we show that any mapping function gives k-approximation retraction, where $k$ is the number of anchors or size of $H$. W.l.o.g assume that graph $G$ is connected. 
Here is the argument: 

\begin{lemma}
Any retraction of vertices of graph $G$ to anchors $H$, gives a $k$-approximation retraction for the maximum stretch. 
\end{lemma}

\begin{proof}
We need to show that between any pair of anchors of $H$, there is a path in $H$ that weight of any edge of it is at most $OPT$, where $OPT$ is the maximum value of stretch in optimal retraction.

We prove it by a contradiction argument. Assume that for some pair of anchors $x$ and $y$, there is no path in $H$, that weight of all edges is at most $OPT$. Let graph $H'$ be a graph obtained by removing all edges of $H$ that have weight greater than $OPT$. From the assumption $H'$ is disconnected and vertex $x$ and $y$ are in different components $S, V(H)-S$. 

Let $\phi$ be the optimal retraction function. Since graph $G$ is connected, there is a path $P: v_0 = x, v_1, ... v_i = y$ which connects $x$ to $y$. There is some edge $(v_j, v_{j+1})$ on $P$ that $\phi(v_j)$ and $\phi(v_{j+1})$ belong to component $S$ and $V(H)-S$ respectively. The stretch of edge $(v_j, v_{j+1})$ is $dist_H(\phi(v_j), \phi(v_{j+1}))$. Since $H'$ is disconnects $\phi(v_j)$ and $\phi(v_{j+1})$, it is the case that $dist_H(\phi(v_j), \phi(v_{j+1})) > OPT$, which is a contradiction that stretch of any edge of $G$ is at most $OPT$.  
\end{proof}



==> problems.tex <==
\newcommand{\GraphRetract}{{\sc GraphRetract}}
\newcommand{\MetricRetract}{{\sc MetricRetract}}

\section{Problem Definition}
In this section, we define the graph and metric retraction problems.  We present their definitions for general hosts; the focus of this paper is on the case where the host forms a uniform cycle. 
\begin{definition}
Given an unweighted {\em guest}\/ graph $G = (V,E)$ and a {\em host}\/ subgraph $H = (A, E')$ of $G$, a mapping $f: V \rightarrow A$ is a retraction of $G$ to $H$ if $f(v) = v$ for all $v \in A$.  For a given retraction $f$ of $G$ to $H$, define the {\em stretch}\/ of an edge $e = (u,v) \in E(G)$ to be $d_H(f(u), f(v))$, where $d_H$ is the distance metric induced by $H$, and the {\em stretch}\/ of $f$ to be the maximum stretch over all edges of graph $G$.  The goal of the {\em minimum graph retraction}\/ problem \GraphRetract\ is to find a retraction of $G$ to $H$ with minimum stretch. 
\end{definition}


In both \GraphRetract\ and \MetricRetract, we focus our attention on the special case where the host forms a uniform cycle; so in \GraphRetract\ $H$ is a cycle in $G$, while in \MetricRetract, $d_H$  is a uniform cycle over $|A|$ points.  In both problems, we refer to the vertices of $A$ as {\em anchors}. 

==> retraction_to_metric.tex <==
\section{Retraction to Metrics (Most likely Omitted)}

\input{k_approximation}

\input{hardness_res}

\subsection{Reducing Graphical metric retraction to Graph retraction}

In this section, we provide a reduction from graphical metric retraction problem to graph retraction problem. Graphical metric is a metric captured by distances of an unweighted graph. 

In graphical metric retraction problem, a metric or distance function is defined over a set $V$ of vertices, and a subset $A$ of $V$ are called anchors. The goal is to map all vertices to anchors subject to minimizing maximum stretch. In graph retraction problem, the goal is to map vertices of the graph to a connected subset of its vertices. The difference between graphical metric retraction and graph retraction is that in graph retraction the distances of subgraph where vertices are mapped to can be different from their distances in original graph, while in graphical metric retraction distances of anchors are based on the distances in original metric. 

Let $G$ be a graphical metric which is defined over a set of vertices $V$, and let set $A \subset V$  be set of anchors. 
Let $G_k$ be the union of all direct shortest paths between any pair of anchors of distance at most $k$, for some arbitrary $k$ at least $1$. By a direct path between a pair of anchors, we mean a path  which none of the intermediate (excluding the endpoints) vertices of the path are anchors.   

In the following, we describe an algorithm that reduces graphical metric retraction problem to graph retraction problem.

\begin{algorithm}
\begin{algorithmic}
\Input {Graphical metric $G$ and $k \geq 1$}
\Output {Embedding function $F$}
  %\SetKwInOut{Output}{Output}
\State {Build graph $G_k$ from $G$ }
\State {Let $E_k$ be the optimal embedding function of $G$ to $G_k$}
\State {Let $F = E_k$}
\For {vertex $v \in V$}
\If {$E_k(v)$ is a non-anchor vertex}
\State { Set $F(v)$ to an anchor vertex which is closest to $E_k(v)$ }\\
        \Comment {(closest with respect to distances in $G_k$)}
     \EndIf
\EndFor \\
\Return F
\end{algorithmic}
\end{algorithm}

\begin{theorem}
If graphical metric $G$ has an optimal embedding of stretch $k$ to its anchors, then embedding function $F$ gives a stretch of at most $2k$. 
\end{theorem}

\begin{proof}
First, we prove that stretch of embedding function $E_k$, the optimal embedding function of $G$ to $G_k$  is at most $k$. Let function $E$ be the optimal embedding function of graphical metric $G$ to its anchor set. From the assumption, stretch of $E$ is $k$. Apply embedding function $E$ for embedding $G$ to $G_k$. Consider an arbitrary adjacent pair of vertices, $u , v \in V$. %($(u,v) \in E(G) $). 
Let $a_u = E(u)$ and $a_v = E(v)$. Since the embedding function $E$ has stretch $k$, this means that $d_G(a_u, a_v) \leq k$. Also $d_{G_k}(a_u, a_v) \leq k$, by $G_k$'s construction. Thus function $E$ has stretch at most $k$ for embedding $G$ to $G_k$. This implies that stretch of $E_k$, the optimal embedding function of $G$ to $G_k$ is at most $k$. 

Second, we prove that stretch of embedding function $F$ is at most $2k$. For an arbitrary adjacent pair of vertices $u,v \in V$, let $a'_v = E_k(v)$ and $a'_u = E_k(u)$, then $d_{G_k}(a'_u, a'_v) \leq k$. If $a'_u$ (similarly $a'_v$ ) is a non-anchor vertex, then by $G_k$'s construction, there should be a direct shortest path $P_u$ in $G_k$ between two anchors such that $a'_u$ lies on it, and length of $P_u$ is at most $k$ by $G_k$'s construction.
In this case, the algorithm set $F(u)$ to closest anchor to $a'_u$ according to distances on $G_k$. Note that distance of $a'_u$ to the closest endpoints of $P_u$ is at most $k/2$. Now $d_{G}(F(u), F(v)) \leq d_{G_k}(F(u), F(v))\leq  d_{G_k}(F(u), a'_u) + d_{G_k}(a'_u, a'_v) + d_{G_k}(a'_v, F(v)) \leq k/2 + k + k/2 = 2k$. This completes the proof that stretch of $F$ is at most $2k$. 

\end{proof}

